Exploring Foundation Models Fine-Tuning for Cytology Classification

Cytology slides are essential tools in diagnosing and staging cancer, but their analysis is time-consuming and costly. Foundation models have shown great potential to assist in these tasks. In this paper, we explore how existing foundation models can be applied to cytological classification. More particularly, we focus on low-rank adaptation, a parameter-efficient fine-tuning method suited to few-shot learning. We evaluated five foundation models across four cytological classification datasets. Our results demonstrate that fine-tuning the pre-trained backbones with LoRA significantly improves model performance compared to fine-tuning only the classifier head, achieving state-of-the-art results on both simple and complex classification tasks while requiring fewer data samples.

==> comments/comments_intro.tex <==

% An effective approach involves using deep learning models to automate classification. 
% This process requires a patch-based method, dividing gigapixel slides into thousands of smaller patches suitable for model training, as handling large-scale cytology images demands high computational resources~\cite{Zhang_2017}. %,SHI2021105807,RAHAMAN2021104649
% It is well-known that the performance of these models is highly dependent on the quantity and diversity of data \cite{Gong_2019}. However, annotating thousands of cytological images is cumbersome and challenging as it must be performed by trained medical practitioners and takes a considerable amount of time~\cite{JIANG2023102691}. As a result, the community is exploring ways to make use of fewer labeled data effectively, an area of research known as few-shot learning \cite{song2022fsl}. \\


% To tackle data scarcity issue, the medical imaging community has started to explore the potential of large-scale foundation models developed through extensive pre-training on large datasets~\cite{Zhang2024biomedclip,caron2021emerging,oquab2023dinov2,Chen2024uni}. These models are valued for their robust generalization capabilities, especially in few-shot settings, aligning well with the medical field's needs. %The benefits of these foundation models align well with the medical field's needs, considering the high cost of annotating medical data. 
%CLIP, a vision-language model (VLM), is one example of these models, that learns to align vision and text embeddings in a common embedding space on large-scale image-text datasets. The creation of large medical datasets has led to the emergence of several medical imaging oriented foundation models~\cite{Zhang2024biomedclip}. 

% Aligning well with medical field's needs, large medical datasets are created, giving rise to the emergence of several medical imaging oriented foundation models~\cite{Zhang2024biomedclip,huang2023plip,Oluchi2023quilt,Lu2024conch,Chen2024uni,eslami2021doesclipbenefitvisual} that have been explored in several studies~\cite{zanella2024boostingvlms,ding2024}.

% We show that using LoRA enhances the fine-tuning of foundation models for cytology tasks, resulting in better performance, even in few-shot settings. \\

    % \item The use of LoRA allows fine-tuning foundation models for cytology with a limited dataset while improving performance.

    % \item CLIP, fine-tuned with LoRA, achieve state-of-the-art results on challenging tasks, using only 70\% of the dataset and reducing the number of trainable parameters by a factor of 62 compared to the current state-of-the-art model.


% \noindent \textcolor{olive}{\textit{Importance of good Cyto classification}}
\begin{comment}
Cytology slides are vital for diagnosing and staging cancer, offering detailed views of abnormal cells to guide treatment decisions~\cite{shaw2000history}. Analyzing these slides is labor-intensive and costly, leading to delays in the reporting process. In clinical settings, cytopathologists also suffer from inter-observer variations~\cite{darragh2013interrater}, making automation essential to improve both classification efficiency and accuracy. \\

% \noindent \textcolor{olive}{\textit{Patch approach and lack of labeled Cyto data}}

An effective approach involves using Deep Learning (DL) models to automate classification. This process requires a patch-based method, dividing gigapixel slides into thousands of smaller patches suitable for model training~\cite{Zhang_2017,SHI2021105807,RAHAMAN2021104649}. However, annotating thousands of patches is cumbersome and challenging for medical practitioners. As a result, the community is exploring ways to make use of fewer labeled data effectively. \\

% \noindent \textcolor{olive}{\textit{Fond. models / VLMs and their success in medical imaging}}

To tackle this challenge, the medical imaging community has started to explore the potential of large-scale foundation models (FMs) developed through extensive pre-training, mainly in the computer vision community~\cite{caron2021emerging,oquab2023dinov2,Chen2024uni}. These models are valued for their robust generalization capabilities, especially in zero-shot and few-shot settings. The benefits of these FMs align well with the medical field's needs, considering the high cost of annotating medical data and inter-observer variability. Among these models, vision-language models (VLMs) like CLIP have demonstrated great potential in zero-shot and few-shot classification, even surpassing supervised competitors in some cases~\cite{Radford2021clip}. Based on contrastive learning to train vision and text embeddings on large-scale image-text datasets, this multi-modal approach can be extended to clinical settings, where text descriptions of images are common. This has led to the emergence of several medical imaging oriented VLMs~\cite{Zhang2024biomedclip,huang2023plip,Oluchi2023quilt,Lu2024conch}. \\

% \noindent \textcolor{olive}{\textit{Few-shot adaptation of VLMs}}

Building on this potential, few-shot adaptation of VLMs has been shown to enhance generalization with minimal labeled data~\cite{zhou2022learning,zhang2022tip,zhu2023prompt}. Traditionally, fine-tuning these models relies on computationally intensive methods like prompt-learning~\cite{zhou2022learning} and adapter-based approaches~\cite{zhang2022tip}. However, recent efficient approaches~\cite{zanella2024cliplora}, based as Low-Rank adaptation~\cite{hu2021lora}, reduce the need for extensive hyperparameter searches and improve the deployability potential of VLM fine-tuning real-world applications such as medical imaging. \\

% \noindent \textcolor{olive}{\textit{Contributions}}

In this work, we explore the few-shot adaptation capabilities of various FMs for cytology classification. We evaluate two vision and three vision-language models pre-trained on natural and biomedical images, comparing their fine-tuning performance on four cytology classification benchmark datasets. We observe that:

\begin{itemize}
    \item Fine-tuning the backbone improves performance and reduces the need for large training sets. %Large-scale vision-language models outperform (learn faster ?) large-scale vision models when it comes to cytology classification.
    \item With optimized LoRA parameters, we successfully reach state-of-the-art results for challenging tasks while using only a small portion of the dataset. %Among all vision-language models considered, CLIP shows better performance (more efficient adaptation?) on cytology classification, even surpassing models pre-trained on various types of medical images.
\end{itemize}
\end{comment}


==> comments/comments_rw.tex <==

\begin{comment}
Over the past few years, DL has garnered increasing attention in the field of cytology. Zhang \textit{et al.}~\cite{Zhang_2017} demonstrated in their work that deeper networks, pre-trained on ImageNet and fine-tuned with cytology datasets, outperformed smaller networks without pre-training in terms of accuracy. This finding has been supported by many cytology classification studies that rely on CNN models pre-trained on ImageNet as feature extractors. These studies typically fine-tuned only the classification layer on top of the backbone to adapt to cytology-specific tasks~\cite{Jiang2023,Jiang2023_review}. The use of pre-trained models has become standard practice in this domain. In a comparative study~\cite{UCAn2022}, the authors evaluated widely-used CNN architectures to classify benign and malignant cells from body fluid cavity cytologies\cite{kaggle2022bodycavity}. Their experiments revealed that ResNet50 achieved an impressive accuracy of 99\%, further highlighting the effectiveness of pre-trained networks in cytological image classification tasks. Another approach proposed in \cite{Yaman2022} introduced a pyramid deep feature extraction method to classify cervix cytological images. This method leveraged transfer learning with DarkNet19 to extract 21,000 features, followed by Neighborhood Component Analysis to select the 1,000 most informative features. These features were then classified using an SVM, achieving 98.26\% accuracy on the SIPaKMeD dataset~\cite{Plissiti2018sipakmed} and 99.47\% on the Mendeley LBC dataset~\cite{Hussain2020}. \\

While CNN models dominate the cytology domain, the recent emergence of transformer-based models is noteworthy. Cai \textit{et al.}~\cite{cai2024hicervix} introduced a hierarchical classification model, HierSwin, also based on a Swin Transformer architecture. This model effectively captured intricate feature relationships across hierarchical levels, achieving a top-1 accuracy of 78.4\% at classification levels 2 and 3 of the HiCervix dataset. Other vision transformer (VT) based models have been explored in the literature albeit briefly, demonstrating promising results~\cite{Jiang2023_review, Jiang2023}.\\

% In \cite{Jiang2023_review, Jiang2023}, transformers like Swin and DeiT have been explored, albeit briefly, demonstrating promising results. For instance, the CVM-Cervix model, which combines CNN with a tiny DeiT, achieved 91.72\% accuracy on a combined SIPaKMeD and Cric datasets (11 classes) and 92.35\% accuracy on the Herlev test set. This hybrid model proved more efficient than either CNN or Vision Transformer (VT) models alone.

More recently, there has been growing interest in few-shot learning techniques for medical imaging tasks. It addresses the challenge of limited labeled data, which is often the case in medical datasets. For instance, the work in \cite{Pachetti2024} explored a novel few-shot learning approach that integrates contrastive learning and meta-learning to improve model generalization on small datasets. Their approach demonstrated strong performance on cytology datasets with minimal training samples, significantly reducing the need for extensive labeled data and making it highly applicable in clinical settings.

% The Swin Transformer, with its shifted window design, creates connections among consecutive layers, while DeiT introduces distillation tokens, reducing the need for extensive datasets and computational resources.

% Furthermore, DeepCervix~\cite{10.1016/j.patcog.2022.108829}, which employed a late fusion of features from four CNNs along with data augmentation, set a new state-of-the-art in cervical cytology classification. It achieved classification accuracies of 99.85%, 99.38%, and 99.14% for 2-class, 3-class, and 5-class tasks, respectively, on the SIPaKMeD dataset. Similarly, DeepPAP, which fine-tuned a ConvNet pre-trained on ImageNet, demonstrated a high accuracy of 98.3% on the Herlev dataset, underscoring the continued relevance and success of transfer learning strategies in cytology~\cite{Zhang_2017}.


% Non-few-shot setting:~\cite{SHI2021105807,RAHAMAN2021104649}

% https://arxiv.org/abs/2404.06080: Few-shot + use of ViT, meta-learning no PEFT 

% "We evaluate models pre-trained on natural and biomedical images, comparing zero-shot learning and fine-tuning while pointing to their effectiveness and limitations in mammographic analysis"
\end{comment}


\begin{comment}
Following the introduction of the first FMs, larger specialized datasets have been developed, leading to the emergence of FMs tailored to specific tasks and domains.
%Examples include UNI~\cite{Chen2024uni}, a FM pre-trained on 100 million pathological images; BiomedCLIP~\cite{Zhang2024biomedclip}, a VLM trained on the largest multimodal biomedical dataset; and QUILT~\cite{Oluchi2023quilt}, a CLIP model fine-tuned on the largest histopathological image-text dataset. 
Examples include the VLMs BiomedCLIP~\cite{Zhang2024biomedclip}, and QUILT~\cite{Oluchi2023quilt}, each specialized for biomedical and histopathological tasks, respectively. UNI~\cite{Chen2024uni} is another VT designed for histopathology. To the best of our knowledge, no FM has yet been introduced specifically for cytological tasks. \\

Adapting FMs, which consist of a large number of parameters, through full fine-tuning typically requires extensive datasets and computational resources. To alleviate these demands, parameter-efficient fine-tuning (PEFT) methods have been developed. These methods allow fine-tuning by training only a small subset of parameters while keeping the majority of the model’s parameters frozen. PEFT methods can be broadly categorized into four groups based on the parameters being trained. Selective fine-tuning methods focus on updating only a subset of the model’s existing weights, while adapter-based methods introduce additional trainable parameters. Another approach, prompt-tuning \cite{zhou2022learning}, replaces hand-designed text tokens with trainable ones for VLMs. Finally, Low-Rank Adaptation (LoRA) \cite{hu2021lora} models weight updates using low-rank matrices. Zanella \textit{et al.}~\cite{zanella2024cliplora} apply LoRA to CLIP, demonstrating that it outperforms both adapter-based and prompt-tuning methods for fine-tuning on natural images, leading to higher performance on average. Similarly, Dutt \textit{et al.}~\cite{dutt2023parameter} evaluated various PEFT methods across transformer-based models on different medical tasks and modalities. Their findings showed that LoRA consistently outperformed full fine-tuning, particularly in low-data scenarios, making it the most effective PEFT method across all datasets tested.

% In their paper, Zanella \textit{et al.}~\cite{zanella2024cliplora} implemented LoRA on the CLIP model~\cite{Radford2021clip} concentrating specifically on the query, key, value and output matrices of the attention block, in both visual and textual encoders. Based on this work, we can apply the same technique on other transformer-based models.

% In the cytological field, to the best of our knowledge, no VLM has been introduced yet. However, \cite{huang2024efficientframeworkbasedlarge} fine-tuned a large foundation model pre-trained on ImageNet with a PEFT adapter-based method on the entire training set to develop a feature extractor specifically for cervical cytopathology.
\end{comment}



% \subsection{Foundation models fine-tuning} 
% One of the earliest FM is the vision transformer introduced by Google~\cite{wu2020visual}. Beyond vision, FMs have been developed  for multiple modalities, including vision and language. Vision-language models, such as CLIP~\cite{Radford2021clip}, learn to align visual and textual embedding in a common embedding space using large-scale image-text datasets. Following the introduction of the first FMs, increasingly specialized datasets have been developed, leading to the emergence of domain-specific FMs. Examples include the vision-language models BiomedCLIP~\cite{Zhang2024biomedclip} and QUILT~\cite{Oluchi2023quilt}, focusing on biomedical and histopathological applications, respectively, as well as UNI~\cite{Chen2024uni}, a vision transformer also designed for histopathology. To the best of our knowledge, no FM has yet been introduced specifically for cytology.

% As fine-tuning these models requires extensive datasets and computational resources, parameter-efficient fine-tuning methods have been developed to train only a small subset of parameters. Among these methods, Low Rank Adaptation (LoRA)\cite{hu2021lora} updates models weight using low-rank matrices. Dutt \textit{et al.}~\cite{dutt2023parameter} evaluated various parameter-efficient fine-tuning methods on transformer-based models on different medical tasks and modalities. Their findings show that LoRA consistently outperforms full fine-tuning, especially in low-data scenarios, establishing it as the most effective parameter-efficient fine-tuning method across all tested datasets.


% V1 =  Many cytology classification studies rely on pre-trained CNN models used as feature extractors. These studies typically fine-tune only the classification layer added on top of the backbone to adapt it to cytology~\cite{Jiang2023,Jiang2023_review}. In a comparative study, Uçan \textit{et al.}~\cite{UCAn2022} test widely-used pre-trained CNN architectures, finding that ResNet50 achieves 99\% accuracy in classifying body cavity cytologies. Another approach proposed by Yaman \textit{et al.}~\cite{Yaman2022} uses DarkNet19 to extract features from cervix cytological images. Combined with machine learning algorithms, they achieve 98.26\% accuracy on the SIPaKMeD dataset~\cite{Plissiti2018sipakmed} and 99.47\% on the Mendeley LBC dataset~\cite{Hussain2020}. However, it is important to note that these are relatively simpler classification tasks, and higher complexity challenges in cytology remain unresolved.

% V2 = Many cytology classification studies rely on pre-trained CNN models used as feature extractors, typically fine-tuning only the classification layer added on top of the backbone~\cite{Jiang2023, Jiang2023_review}. Uçan \textit{et al.}~\cite{UCAn2022}, for example, compared various CNN architectures, identifying widely-used models like ResNet50 as effective classifiers for body cavity cytologies. Another approach by Yaman \textit{et al.}~\cite{Yaman2022} employs DarkNet19 to extract features from cervix cytological images, combining it with traditional machine learning techniques. While CNNs remain prevalent in cytology, transformer-based models have recently gained attention for their ability to capture complex feature relationships, delivering promising results~\cite{Jiang2023_review, Jiang2023}. Cai \textit{et al.}~\cite{cai2024hicervix} introduce a hierarchical classification model, HierSwin, based on a Swin Transformer architecture, which leverages hierarchical information across levels, marking a shift toward more intricate transformer architectures for cytology.


